Unlimited Lives: Secure In-Process Rollback with Isolated Domains

The use of unsafe programming languages still remains one of the major root causes of software vulnerabilities. Although well-known defenses that detect and mitigate memory-safety related issues exist, they don't address the challenge of software resilience, i.e., whether a system under attack can continue to carry out its function when subjected to malicious input. We propose secure rollback of isolated domains as an efficient and secure method of improving the resilience of software targeted by run-time attacks. We show the practicability of our methodology by realizing a software library for Secure Domain Rollback (SDRoB) and demonstrate how SDRoB can be applied to real-world software.

==> Makefile <==

ISPELLPAT = -ktexskip1 +cref,Cref,url,todo,presetkeys,newcommand,definecolor


all: main.pdf

main.pdf: *.tex sections/*.tex
	latexmk -pdflatex='pdflatex -file-line-error' -pdf main.tex

spelling: *.tex sections/*.tex
	for file in *.tex sections/*.tex; do \
          ispell -t ${ISPELLPAT} -b -d american -p ./paper.dict $$file; \
        done

clean:
	latexmk -C -pdflatex='pdflatex -file-line-error' -pdf main.tex
	rm -f main.pdf
	rm -f *.tex.bak

distclean: clean
	rm -f main.bbl



==> sections/csx.tex <==
%\enlargethispage{1em}
%
We implement the concept of secure domain rollback as \emph{\SDRoB} -- a 
C-language Linux library for the 64-bit x86 architecture using PKU as the
underlying isolation primitive. The library provides an API to control the life
cycle of domains.
%Below we describe this API and the
%implementation of \SDRoB.

\begin{table}
    \footnotesize
    \caption{\label{Tab:sdrobapi} \SDRoB API.  udi: user domain index.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l | l|  l|}
    \hline 
     API Name  &  Arguments & Description\\   
     \hline\hline
     \hspace{-.5em}\dCOne \texttt{sdrob\_init()}   & udi, options      & Initialize Domain \emph{udi}  \\
     \hline 
     \hspace{-.5em}\dCTwo \texttt{sdrob\_malloc()}  & udi, size & Allocate \emph{size} memory in domain \emph{udi}  \\  
     \hline 
     \hspace{-.5em}\dCThree \texttt{sdrob\_free()}  & udi, adr & Free memory at \emph{adr} in domain \emph{udi}  \\  
     \hline 
     \hspace{-.5em}\dCFour \texttt{sdrob\_dprotect()}&  udi, tddi,  & Set domain \emph{udi}'s access permissions \\
                                        &  PROT                & to \emph{PROT} on target data domain \emph{tddi} \\
     \hline 
     \hspace{-.5em}\dCFive \texttt{sdrob\_enter()}   & udi      & Enter Domain \emph{udi} \\
     \hline 
     \hspace{-.5em}\dCSix \texttt{sdrob\_exit()}  &  ---          & Exit Domain \emph{udi} \\
     \hline 
     \hspace{-.5em}\dCSeven \texttt{sdrob\_destroy()}  & udi, options & Destroy Domain \emph{udi}\\
     \hline     
     \hspace{-.5em}\dCEight \texttt{sdrob\_deinit()}  & udi & Delete return context of Domain \emph{udi}\\
     \hline     
     \hspace{-.5em}\dCNine \texttt{sdrob\_call()}    & udi, fun, arg,& Convenience wrapper for single \\ 
                                        & size, ret  & function calls with one argument\\
     \hline
    \end{tabular}}
\end{table}

\subsection{\SDRoB API} 
\label{sec:api}
Developers use the \SDRoB API calls shown in \Cref{Tab:sdrobapi} to
flexibly enhance
their application with a secure rollback mechanism, accounting
for the design patterns described above.

Domains are initialized by \texttt{sdrob\_init()} \dCOne where the developer
chooses a unique index to reference the domain in future API
calls. \emph{Execution} and \emph{data} domains may be created, where the latter
may hold shareable data but cannot execute code. For execution domains we
further distinguish domains that are \emph{\nonisolated} or \emph{\isolated}
to their parent, and whether an abnormal domain exit should be handled in the
parent or grandparent domain. A domain can only be initialized once per thread
(unless it is deinitialized or destroyed before by the programmer) and the point
of initialization for execution domains marks the execution context to which
control flow returns in case of an abnormal domain exit.

The API call's return value fulfills two roles. When the domain is first
initialized, it returns \emph{OK} on success or an error message, e.g.,
% due to
% misconfiguration or
if the domain was already initialized in the current
thread. On abnormal domain exit, control flow returns another time from the
init function and the return value signifies the index of the nested domain that
failed and was configured to return to this point. This means that error
handling for abnormal domain exits needs to be defined in a case split on the
return value of the \texttt{sdrob\_init()} function.

After initialization, memory in an execution or data domain can be managed
using \texttt{sdrob\_malloc()} \dCTwo and \texttt{sdrob\_free()} \dCThree, e.g.,
to be able to pass arguments into the domain. Note that this is only allowed for
child domains of the current domain that are \nonisolated. For \isolated
domains, a shared data domain needs to be used to exchange
data. Using \texttt{sdrob\_dprotect()} \dCFour access permissions to a data
domain can be configured for child domains.

An execution domain initialized in the current domain can be entered
and exited using \texttt{sdrob\_enter()} \dCFive and \texttt{sdrob\_exit()}
\dCSix. This switches the stack and heap to the selected domain and back, and
changes the memory access permissions accordingly. Currently, the \SDRoB
prototype does not copy local variables on such domain transitions. Such
variables need to be passed via registers or heap memory.

Supporting the transient domain design pattern, child domains can be deleted
using \texttt{sdrob\_destroy()} \dCSeven \ifabridged . \fi \ifnotabridged, with the option to either discard the
domain's heap memory or, if \nonisolated, merge it to the current domain.\fi The
persistent domain pattern can then be implemented by simply not destroying the
domain after exiting it, so that it can be entered again.

An important requirement is that a nested execution domain needs
to be destroyed before the function that initialized that domain
returns. Otherwise, the stored execution context to which to return to would
become invalid as it would point to a stack frame that no longer exists. To
provide more flexibility, \texttt{sdrob\_deinit()} \dCEight
allows to just discard a child domain's execution context but leave its memory
intact. Before entering the domain again, it needs to be re-initialized, setting
a new return context for abnormal exits.

Finally, we provide \texttt{sdrob\_call()} \dCNine which
implements the life cycle of \texttt{enter\_domain()} shown
in \Cref{fig:sdroblifecycle} for a function $F$ that receives a pointer to an
object in memory as input and returns an integer-sized value. To illustrate the
API, \Cref{lst:sdrob_call} shows how \texttt{sdrob\_call()} can be implemented.

\ifnotabridged
\begin{lstlisting}[style=CStyle, float, belowskip=-0.8 \baselineskip, escapechar=@@, label={lst:sdrob_call}, caption={Pseudocode showing a possible implementation of \texttt{sdrob\_call(udi\_F,F,arg,size,ret)} using other API calls (orange).}]
int err = sdrob_init(udi_F, EXECUTION_DOMAIN | 
                     ACCESSIBLE | RETURN_HERE);
if (err == OK ){
   // prepare passing return value and argument
   register int r asm ("r12");
   register void *adr asm ("r13");
   adr = sdrob_malloc(udi_F, size); 
   if (!adr && size>0) { return MALLOC_FAILED; }   
   if (size>0) { memcpy(adr, arg, size); }
   sdrob_enter(udi_F); 
   // invoke F on copy of argument and save return value
   r = F(adr);
   sdrob_exit();
   if (ret) { *ret = r; }
   sdrob_free(adr);
   sdrob_destroy(udi_F, NO_HEAP_MERGE);
}
return err;
\end{lstlisting}
\fi
\ifabridged
\begin{lstlisting}[style=CStyle, float, belowskip=-0.8 \baselineskip, escapechar=@@, label={lst:sdrob_call}, caption={Pseudocode showing a possible implementation of \texttt{sdrob\_call(udi\_F,F,arg,size,ret)} using other API calls (orange).}]
    int err = sdrob_init(udi_F, EXECUTION_DOMAIN | 
                         ACCESSIBLE | RETURN_HERE);
    if (err == OK ){
       // prepare passing return value and argument
       register int r asm ("r12");
       register void *adr asm ("r13");
       adr = sdrob_malloc(udi_F, size); 
       if (!adr && size>0) { return MALLOC_FAILED; }   
       if (size>0) { memcpy(adr, arg, size); }
       sdrob_enter(udi_F); 
       // invoke F on copy of argument and save return value
       r = F(adr);
       sdrob_exit();
       if (ret) { *ret = r; }
       sdrob_free(adr);
    \ifnotabridged
       sdrob_destroy(udi_F);
    \fi
    }
    return err;
\end{lstlisting}
\fi

In the example, we first initialize a new \nonisolated execution domain for
function \emph{F}. If an abnormal exit occurs in that domain,
control returns here, so we save the error code in \texttt{err}. If
initialization succeeded, we allocate a local variable \texttt{r} in a register
to retrieve the return value later. We also allocate memory for the input
argument at \texttt{adr} in the new domain. Since that domain is \nonisolated,
we can copy the argument directly from the parent domain. Afterwards, we enter
the nested domain and invoke \emph{F} on the copy of the argument, saving the
return value. After exiting, we are back in the parent domain and can copy the
return value to the desired location (which is inaccessible to the nested
domain). We free all temporary memory and destroy the nested domain, freeing its
remaining memory.\footnote{Calling \texttt{sdrob\_free()} is actually
redundant here; \texttt{sdrob\_destroy()} would free this memory as well
\ifnotabridged with the \texttt{NO\_HEAP\_MERGE} option \fi.}  Finally, we
return \texttt{OK} in case of normal domain exit, or the error code
otherwise. Users of \texttt{sdrob\_call()} can then define their own error
handling depending on this return value as shown earlier.

\begin{figure*}
\noindent\begin{minipage}{\textwidth}
\begin{lstlisting}[style=CStyle, belowskip=-0.8 \baselineskip, label={lst:openssl_wrapper}, caption={excerpt from wrapper function for \texttt{EVP\_EncryptUpdate()} that executes OpenSSL in a persistent nested domain. Data is passed between the parent and nested domain via a distinct shared data domain (\texttt{OPENSSL\_DATA\_UDI}). Error handling is omitted in excerpt for brevity.}]
int __wrap_EVP_EncryptUpdate(EVP_CIPHER_CTX *ctx %*\hspace{-.5em}\dOne\hspace{-.5em}*), unsigned char *out, int *outl, const unsigned char *in, int inl) {
    register evp_encrypt_update_args_t *args asm ("r12");%*\footnotemark*)  // holds copied function arguments and return value
    %*$\ldots$ *)
    args = sdrob_malloc(OPENSSL_DATA_UDI, sizeof(evp_encrypt_update_args_t)); %*\dTwo*)
    args->ctx = ctx; %*\dTwo*)                       // copy ctx from current domain to shared data domain
    args->inl = inl; %*\dTwo*)                       // copy inl from current domain to shared data domain
    %*\tikzmark{obegin}*)
    if (out != NULL && inl >= 0) {            // inl + cipher_block_size is upper bound for yet unknown output size 
        args.out = sdrob_malloc(OPENSSL_DATA_UDI, inl + cipher_block_size%*\footnotemark*));
    } else { args.out = NULL; }
    %*\tikzmark{oend}*)                                             %*\tikzmark{ocomment}*)
    %*\tikzmark{ibegin}*)
    if (in != NULL && inl >= 0) {
        args->in = sdrob_malloc(OPENSSL_DATA_UDI, (size_t)inl);
        memcpy(args->in, in, inl);            // copy in from current domain to shared data domain
    } else { args.in = NULL; }
    %*\tikzmark{iend}*)                                             %*\tikzmark{icomment}*)
    sdrob_enter(OPENSSL_UDI);                 // execute real EVP_EncryptUpdate in inaccessible domain
    args->ret = __real_EVP_EncryptUpdate(args->ctx, args->out, &(args->outl), args->in, args->inl);
    sdrob_exit();
    %*\tikzmark{cbegin}*)
    *outl = args->outl;                       // copy out outl value from shared data domain
    if (out != NULL) {                        // copy out encrypted data from shared data domain
        memcpy(out, args->out, (size_t)*outl);
    }
    %*\tikzmark{cend}*)                                             %*\tikzmark{ccomment}*)
    %*$\ldots$*)
}
\end{lstlisting}
\begin{tikzpicture}[remember picture, overlay, thick]
    \draw[decorate,decoration={brace,amplitude=5pt,mirror}] ([shift={(-4pt,-2pt)}]pic cs:obegin) 
    -- ([shift={(-4pt,5pt)}]pic cs:oend) 
    coordinate[midway,xshift=-6pt](Btip);
    \draw[->, rounded corners] (Btip) -- +(-4pt,0) |- (pic cs:ocomment) node[right,comment,thin]
    {\scriptsize \dThree Set up output buffer. Replaced with \texttt{args.out = out} if \texttt{out} points to shared data domain.};

    \draw[decorate,decoration={brace,amplitude=5pt,mirror}] ([shift={(-4pt,-2pt)}]pic cs:ibegin) 
    -- ([shift={(-4pt,6pt)}]pic cs:iend)
    coordinate[midway,xshift=-6pt](Btip);
    \draw[->, rounded corners, bend left=45] (Btip) -- +(-4pt,0) |- ([yshift=4pt]pic cs:icomment) node[right,comment,thin]
    {\scriptsize \dFour Set up input buffer. Replaced with \texttt{args.in = in} if \texttt{in} points to a readable domain.};

    \draw[decorate,decoration={brace,amplitude=5pt,mirror}] ([shift={(-4pt,-2pt)}]pic cs:cbegin) 
    -- ([shift={(-4pt,5pt)}]pic cs:cend) 
    coordinate[midway,xshift=-6pt](Btip);
    \draw[->, rounded corners] (Btip) -- +(-4pt,0) |- (pic cs:ccomment) node[right,comment,thin]
    {\scriptsize \dFive Copy out. Omitted if \texttt{out} points to a shared data domain.};
\end{tikzpicture}
\end{minipage}
\end{figure*}

% \begin{lstlisting}[style=CStyle, float=*, belowskip=-0.8 \baselineskip, label={lst:openssl_wrapper}, caption={excerpt from wrapper function for \texttt{EVP\_EncryptUpdate()} that executes OpenSSL in a persistent nested domain. Function arguments is passed between the parent and nested domain via a distinct shared data domain (\texttt{OPENSSL\_DATA\_UDI}). In and out buffer is allocated from data domain. Error handling is omitted in excerpt for brevity.}]
% int __wrap_EVP_EncryptUpdate(EVP_CIPHER_CTX *ctx %*\hspace{-.5em}\dOne\hspace{-.5em}*), unsigned char *out, int *outl, const unsigned char *in, int inl) {
%     register evp_encrypt_update_args_t *args asm ("r12");%*\footnotemark*)  // holds copied function arguments and return value
%     %*$\ldots$ *)
%     args = sdrob_malloc(OPENSSL_DATA_UDI, sizeof(evp_encrypt_update_args_t)); %*\dTwo*)
%     args->ctx = ctx;     %*\dTwo*)                       // copy ctx from current domain to shared data domain
%     args->out = out; %*\dThree*)  %*\dTwo*)                         // copy out from current domain to shared data domain
%     args->outl = outl;   %*\dTwo*)                      // copy outl from current domain to shared data domain
%     args->in = in;   %*\dThree*)  %*\dTwo*)                         // copy in from current domain to shared data domain
%     args->inl = inl;     %*\dTwo*)                      // copy inl from current domain to shared data domain

%     sdrob_enter(OPENSSL_UDI);                 // execute real EVP_EncryptUpdate in isolated domain
%     args->ret = __real_EVP_EncryptUpdate(args->ctx, args->out, &(args->outl), args->in, args->inl);
%     sdrob_exit();

%     *outl = args->outl; %*\dTwo*)                    // copy out outl value from shared data domain
%     sdrob_free(OPENSSL_DATA_UDI, args);
% }
% \end{lstlisting}

\begin{changed}
\paragraph{OpenSSL}
\Cref{lst:openssl_wrapper} shows an \texttt{EVP\_EncryptUpdate()} wrapper for
OpenSSL that implements the persistent domain pattern introduced in
\Cref{sec:domainlifecycle}. Here, OpenSSL allocates its data, such as the
context (\texttt{ctx}) \dOne from a domain which is \isolated from its parent.
While the caller can hold a pointer to \texttt{ctx}, the object itself is
inaccessible to the parent domain. Arguments are copied in via a data domain (\dTwo).
The wrapped function must read bufferred input and write its output to its parent domain.
There are three possible design choices for passing buffer data between the respective domains: 
\begin{inparaenum}[1)] 
\item the OpenSSL domain has read-only access to the parent, i.e., it's called
from the \rootdomain; input can be read directly, but output must be copied through
the data domain used for argument passing (\dThree, \dFive)
\item the parent domain is inaccessible to the OpenSSL and it must copy both
input and output via the data domain used for argument passing (\dThree,
\dFour, \dFive) \item the parent domain is responsible for setting up a shared
data domain between the respective domains and the wrapper can access the
shared area directly via the argument pointers.    
\end{inparaenum}

This persistent domain can be
combined with a transient domain as shown in \Cref{fig:sdrobrollback} to
\begin{inparaenum}[1)]
    \item encapsulate the pointer to \texttt{ctx} within an outer domain, and
    \item to protect the root domain from errors in the caller, such as an \texttt{out} buffer of insufficient size.
\end{inparaenum}
\Cref{sec:openssl_example} shows a concrete usage example.
\end{changed}

% \begin{changed}
% \Cref{lst:openssl_wrapper} shows a \texttt{EVP\_EncryptUpdate()} wrapper for
% OpenSSL that implements the persistent domain
% pattern introduced in \Cref{sec:domainlifecycle}. Here, OpenSSL allocates it's
% data, such as its context (\texttt{ctx}) \dOne from a domain which is strongly
% isolated from its parent. While the caller can hold a pointer to \texttt{ctx},
% the object itself is unaccessible to the parent domain. \dTwo shows how function argument 
% is allocated and passed to OpenSSL domain area. 
% Functions that enter the domain through such wrappers must receive their input and write their
% output via an intermediate shared data domain \dThree This persistent domain can be
% combined with a transient domain as shown in \Cref{fig:sdrobrollback} to
% \begin{inparaenum}[1)]
%     \item encapsulate the pointer to \texttt{ctx} within an outer domain, and
%     \item to protect the root domain from errors in the caller, such as an \texttt{out} buffer of insufficient size.
% \end{inparaenum}
% \Cref{lst:OpenSSLExample} in \Cref{sec:openssl_example} shows another example usage of the wrapper.
% \end{changed}

% The above listing contains two footnote marks so we need to adjust the footnote
% counter manually before each footnote text to correct the footnote numbering

\subsection{Implementation Overview} 


In a nutshell, \SDRoB is implemented using four components:
\begin{inparaenum}[1)] 
\item a hardware mechanism for enforcing in-process memory protection,
\item an isolated \emph{monitor data domain} that houses control data for managing execution and data domains,
\item initialization code that is run at the beginning of each application that is linked to the \SDRoB library, setting up the monitor domain and memory protection, as well as 
\item trusted reference monitor code that realizes the \SDRoB API calls, having exclusive access to the monitor data domain.
\end{inparaenum}
Below we provide more details about these components.

\paragraph{Memory Protection} 
\SDRoB uses PKU protection keys (cf.~\Cref{sec:mpk}) as a hardware-assisted SFI 
mechanism to create different isolated domains within an application governed by
different memory access policies.  When a domain is created, a unique protection
key is assigned for it. At each domain transition, PKRU is updated to grant
access to memory areas as permitted for the newly entered domain, and to prevent
access to other memory areas.

Our evaluation platform supports Intel PKU, hence it allows us to manage up to
15 isolated domains at a time for each process. Software abstractions for
MPK, like libmpk~\cite{Park19}, increase the number of available domains.

\paragraph{\SDRoB Control Data} 
\SDRoB stores global control data in the monitor data domain for keeping track of,
e.g., the registered domain identifiers and the protection key usage. It also
stores per-thread information for domains such as stack size, heap size, parent
domain, and memory access permissions. To support abnormal domain exits, the
currently executing domain and the saved execution contexts are stored too.

\paragraph{Initialization}  An application is compiled with the \SDRoB 
library to use the rollback mechanism. The library provides a
constructor function that is executed before \texttt{main()} to assign all
application memory to the initial isolated domain as a \rootdomain
associated with one of the PKU protection keys. It then initializes \SDRoB global
control data where the default stack and heap size for domains is configurable
through environment variables. Furthermore, it sets the \rootdomain as active
domain, to be updated at domain transitions by the reference monitor, and
finally initializes a signal handler.  

For the multithreading scenario, \SDRoB has a thread constructor function as
well, that is executed before the thread start routine function to assign a
thread memory area to a domain and associate it with one of the protection keys.


\paragraph{Reference Monitor} 
The reference monitor is responsible for book-keeping of domain information
in \SDRoB control data. It performs domain initialization, domain
memory management, and secure domain transitions, including updating the memory
access policy, and saving and restoring the execution state of the
calling domain. Only the reference monitor has access to the monitor data
domain by updating the PKRU register accordingly. The monitor code is executed
using the stack of the nested domain that invoked it.

\paragraph{Rollback} 
The secure rollback from a domain is achieved by the reference 
monitor saving the execution context of the parent domain into \SDRoB control data
when that domain is initialized. \SDRoB uses a \texttt{setjmp()}-like functionality
to store the stack pointer, the instruction pointer, the values of other
registers, and the signal mask for the context to which the call
to \texttt{sdrob\_init()} returns. Note that we cannot simply
call \texttt{setjmp()} within \texttt{sdrob\_init()} because that execution context
would become invalid as soon as the initialization routine returns. On an
abnormal domain exit, the saved parent execution state can be used by the
recovery process to restore the application’s state to the initialization point
prior to entering the nested domain by using \texttt{longjmp()}. This rollback
allows the application to continue from that last secure point of execution that
is now redirected to the developer-specified error handling code. To simplify
programming under these non-local goto semantics~\cite{setjmp}, we only allow to set the return point once per domain and
thread. Moreover, the convention that a domain needs to be destroyed or
deinitialized before the function that initialized it returns, ensures that the
saved execution context is always valid.

\subsection{Memory Management and Isolation}\label{sec:sdrobisolation}
The secure rollback mechanism is achieved by creating different domains within
an application and ensuring that a memory defect within a domain only affects
that domain's memory, not the memory of others. Using the underlying SFI
mechanism based on PKU, each domain is isolated from other domains.

\paragraph{Global Variables}
We modify the linker script to ensure that global variables are allocated in a
page-aligned memory region that can be protected by PKU.
At application initialization, all global variables are assigned to the
\rootdomain; consequently they are not accessible to nested domains. As a pragmatic
solution to the problem, we make the \rootdomain by default read-only
for all nested domains. Write access to global data may then be achieved by
allocating it on the heap of a shared data domain, referenced by a global
pointer.  Note that this approach breaks the confidentiality of the \rootdomain
towards nested domains. As our main goal is integrity, and confidential data can
still be stored and processed in separate domains, we find it a reasonable
trade-off for our prototype.

\paragraph{Stack Management}
\SDRoB creates a disjoint stack for each execution domain to ensure that the code
running in a nested domain cannot affect the stacks of other domains. The stack
area is allocated when first initializing a domain and protected using the
protection key assigned to that domain. As an optimization, we never unmap the
stack area, even when the domain is destroyed, but keep it for reuse, i.e., when
a new domain is initialized. At each domain entry, we change the stack pointer
to the nested domain stack pointer and push the return address of
the \texttt{sdrob\_enter()} call, so that the API call returns to the call site
using the new stack. Then we update the PKRU register according to memory access
policy for that domain. A similar maneuver is performed when switching back to
the parent domain's stack via \texttt{sdrob\_exit()}.

%
% TN: Background information on glibc malloc(), can be omitted from abridged version
% if tight on space. 
% OPENSSL Example footnote
\addtocounter{footnote}{-1}
\footnotetext{The \texttt{args} pointer is kept in a callee-saved register (\texttt{r12}) to ensure it remains accessible to the nested domain after \texttt{sdrob\_enter()} (line 17) changes the domain stack}
%

\addtocounter{footnote}{+1}
\footnotetext{The \texttt{args.out} buffer requires room to store
\texttt{inl} + \texttt{cipher\_block\_size} bytes of data. The
\texttt{cipher\_block\_size} is known from \texttt{ctx}~\cite{opensslman}.}


\paragraph{Heap Management}
\ifnotabridged
In order to manage a domain's heap allocations as described
in \Cref{sec:domainlifecycle} the underlying allocator must have the
ability to differentiate between allocations that occur in different domains and
ensure that the underlying memory is chosen from an address range in a
particular domain's reserved heap area.  Traditionally the heap is set up to be
one large continuous memory area. Modern \texttt{malloc()}
implementations, including the GNU Allocator in
glibc~\cite{glibc} have the ability to maintain multiple disjoint heap areas, typically
for the purpose of optimizing memory access patterns in multi-threaded
applications. For example, the GNU Allocator internally maintains one or more
memory areas, referred to as \emph{arenas}, that are reserved
via \texttt{mmap()} to provide the backing memory for the application's initial
heap and subsequently allocated thread heaps.  Concurrent allocations require
threads to obtain a lock on the arena structure that \texttt{malloc()} operates
on.  Consequently, by assigning different arenas to different threads the GNU
Allocator enables memory allocations in different threads to occur concurrently
without interfering with each other.  Unfortunately the GNU Allocator's design
does not guarantee thread-isolation between arenas: if a thread fails to
allocate memory from the arena attached to it, the \texttt{malloc()}
implementation continues the search for a suitable large block of memory to
satisfy the allocation from the application's other
arenas~\cite{glibcmalloc}.
\fi
%
%\begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{0.45\textwidth}
%  \centering
%  \includegraphics[width=\textwidth]{figures/sdrobtlsfarchitecture1.pdf}
%  \caption{a}
%  \label{fig:sdrobtlsfarchitecture1}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[b]{0.45\textwidth}
%  \centering
%  \includegraphics[width=\textwidth]{figures/sdrobtlsfarchitecture2.pdf}
%  \caption{b}
%  \label{fig:sdrotlfsarchitecture2}
%  \end{subfigure}
%  \caption{}
%  \label{fig:sdrobtlsfarchitecture}
%\end{figure}
%
%\ifnotabridged\paragraph{TLSF}\fi
Because heap isolation in \SDRoB requires memory management with strict
guarantees that allocations within a domain are satisfied only from memory
reserved for that domain, we opted to use an allocator that natively supports
fully disjoint heap areas instead of the default glibc GNU
Allocator\ifabridged~\cite{glibcmalloc}\fi.
For our %proof-of-concept
implementation, we chose the Two-Level Segregated Fit
(TLSF)~\cite{tlsf} allocator~\cite{mattcontetlsf}.
TLSF is a "good-fit", constant-time allocator that allocates memory blocks from
one or more pools of memory. \ifnotabridged Each free block in a pool is linked in two
different doubly linked lists:
\begin{inparaenum}[1)]
\item a free list of blocks belonging to the same size class, and
\item a list ordered by physical address.
\end{inparaenum}
The TLSF control structure contains a \emph{free list bitmap} that describes the
availability of free memory blocks in different size ranges.  TLSF uses
processor bit instructions and the bitmap to locate a corresponding linked list
of suitable-sized free blocks. \fi

Each \SDRoB domain is an assigned its own TLSF control structure and memory pool that correspond to the domain's subheap.
The size of the initial pool assigned to domains is configurable via an environmental variable.
Each individual TLSF pool is limited to 4GB in size~\cite{tlsf}.
Beyond that, a domain's memory is increased by reserving additional pools for the domain's TLSF allocator.

\paragraph{Lazy Heap Initialization}
In order to reduce the memory footprint when domains don't make heap allocations,
the control structure and initial memory pool are not initialized when the
domain is created.  Instead, the reference monitor initializes the domain's TLSF
instance the first time the domain allocates heap memory with
the \texttt{malloc()} family of functions.
We interpose such functions with wrappers by placing the SDRoB library before libc in the library load order.
Upon initialization the associated memory pool is protected by associating it with the domain's protection key.
\ifnotabridged
\paragraph{Subheap Merging} 
Recall from \Cref{sec:api} that a domain's subheap is either discarded or merged with
the parent domain's subheap when \texttt{sdrob\_destroy()} is called, depending on
the option parameter provided.  To enable subheap merging we extended the TLSF
implementation to associate a partially consumed pool to
a pre-existing TLSF control structure.  When a subheap is merged, its
associated protection key is updated to match the parent domain's protection
key. The parent's TLSF control structure is then updated as follows:
\begin{inparaenum}[1)]
  \item detect used and unused blocks in the memory pool being merged, 
  \item link all these blocks to the pre-existing block lists in the parent domain,
  \item update the parent domain's TLSF free list bitmap for unused blocks, and
  \item delete the child domain's TLSF control structure.
\end{inparaenum}
If the heap is not be merged when the domain is destroyed any allocations are
freed and the underlying memory pools can be reused by new domains.
\fi

\paragraph{Error Detection}
Memory access violations are generally reported to userspace software either via
\begin{inparaenum}[1)]
    \item a \texttt{SEGFAULT} signal, e.g. when a domain tries to access memory
        past the confines of the domain’s memory area, and
    \item calls to runtime functions inserted by instrumentation, e.g., GCC's
        stack protector calls \texttt{\_\_stack\_chk\_fail()} if a stack guard
        check fails. 
\end{inparaenum} The \texttt{\_\_stack\_chk\_fail()} function is typically
provided by glibc and terminates the application.  During process
initialization \SDRoB sets up its own signal handler for the \texttt{SEGFAULT}
signal that attributes the segmentation fault to its cause using the signal code
(\texttt{si\_code}) available via a \texttt{siginfo\_t} structure~\cite{sigaction}
provided by the runtime to the signal handler. For instance, violations of PKU
access rules are reported by \texttt{SEGV\_PKUERR} signal code.
In Linux the \texttt{SEGFAULT} signal is always delivered to the thread that generated it.
If the \SDRoB signal handler detects that a violation occurs in a nested domain
it can trigger an abnormal domain exit. If a segmentation fault occurs in a
\rootdomain, or the fault is attributed to a cause the \SDRoB signal handler
is not prepared to handle the process is still terminated. \SDRoB also provides
its own implementation of \texttt{\_\_stack\_chk\_fail()} that replaces the
glibc implementation to respond to stack guard violations.

\SDRoB can be extended to incorporate other run-time error detection
mechanisms, such as Clang CFI~\cite{cficlang}
or heap-based overflow protections (e.g., heap red zones~\cite{Serebryany19}),
improving the recovery capabilities. Probabilistic and passive protections such
as ASLR hinder the exploitation of memory safety violations but cannot detect
them. Yet, our rollback mechanism is compatible with ASLR, as domains
are created at run-time.


==> sections/performance_ev.tex <==

\todo[inline]{We probably don't need this section?!}


